Bunk8s: Enabling Easy Integration Testing of Microservices in Kubernetes

Microservice architecture is the common choice for cloud applications these days since each individual microservice can be independently modified, replaced, and scaled. However, the complexity of microservice applications requires automated testing with a focus on the interactions between the services. While this is achievable with end-to-end tests, they are error-prone, brittle, expensive to write, time-consuming to run, and require the entire application to be deployed. Integration tests are an alternative to end-to-end tests since they have a smaller test scope and require the deployment of a significantly fewer number of services. The de-facto standard for deploying microservice applications in the cloud is containers with Kubernetes being the most widely used container orchestration platform. To support the integration testing of microservices in Kubernetes, several tools such as Octopus, Istio, and Jenkins exist. However, each of these tools either lack crucial functionality or lead to a substantial increase in the complexity and growth of the tool landscape when introduced into a project. To this end, we present \emph{Bunk8s}, a tool for integration testing of microservice applications in Kubernetes that overcomes the limitations of these existing tools. \emph{Bunk8s} is independent of the test framework used for writing integration tests, independent of the used CI/CD infrastructure, and supports test result publishing. A video demonstrating the functioning of our tool is available from \url{https://www.youtube.com/watch?v=e8wbS25O4Bo}.

==> sections/00_abstract.tex <==
\begin{abstract}

% Better testability is one of the key advantages of following a microservice architectural pattern over a monolithic approach. However, the complexity specific to microservice applications requires automated testing with a focus on the interactions between services. While this is achievable with end-to-end tests, another challenge is using few end-to-end tests in a test suite, since they are error-prone, brittle, expensive to write, and time-consuming to run and require many services to be launched. In this regard, an alternative to end-to-end tests are integration tests, which have a smaller test scope than end-to-end tests and therefore allow for deploying less services.  A popular deployment strategy for microservices are containers, with Kubernetes as the most common container orchestration platform. When testing an application that is deployed to Kubernetes, it is not possible to run integration tests for backend subsystems outside of Kubernetes. This would require either deployment of frontend services or a reconfiguration of Kubernetes. The former would lead to an increased testing scope, while the latter may be not possible since Ingresses only support routing HTTP traffic. Therefore, the only solution is to run integration tests inside the cluster. There already exist tools, that enable running integration tests inside a Kubernetes cluster. However, each of those tools either lack crucial functionality or result in an substantial increase in complexity and growth of the tool landscape when introducing them into a project. In order to enable running integration tests inside of Kubernetes, while compensating for the shortcomings of already existing tools, the testing tool Bunk8s was developed. 

% One of the key advantages of following a microservice architectural pattern over a monolithic approach is better testability. However, the complexity specific to microservice applications requires automated testing with a focus on the interactions between the services. 

Microservice architecture is the common choice for cloud applications these days since each individual microservice can be independently modified, replaced, and scaled. However, the complexity of microservice applications requires automated testing with a focus on the interactions between the services. While this is achievable with end-to-end tests, they are error-prone, brittle, expensive to write, time-consuming to run, and require the entire application to be deployed. Integration tests are an alternative to end-to-end tests since they have a smaller test scope and require the deployment of a significantly fewer number of services. The de-facto standard for deploying microservice applications in the cloud is containers with Kubernetes being the most widely used container orchestration platform. To support the integration testing of microservices in Kubernetes, several tools such as Octopus, Istio, and Jenkins exist. However, each of these tools either lack crucial functionality or lead to a substantial increase in the complexity and growth of the tool landscape when introduced into a project. To this end, we present \emph{Bunk8s}, a tool for integration testing of microservice applications in Kubernetes that overcomes the limitations of these existing tools. \emph{Bunk8s} is independent of the test framework used for writing integration tests, independent of the used CI/CD infrastructure, and supports test result publishing. A video demonstrating the functioning of our tool is available from \url{https://www.youtube.com/watch?v=e8wbS25O4Bo}.

% These days most of the cloud based applications are microservices-based architecture since each individual microservice can be independently scaled, upgraded and replaced. Automated testing of such an application involving many number of microservices would involve interaction between the microservices.
% The standard approach for running integration tests for 

% An alternative to end-to-end tests are integration tests

% A video demonstrating the functioning of our tool is available from \url{https://www.youtube.com/watch?v=e8wbS25O4Bo}.

%Placeholder

% The functional and non-functional requirements on Bunk8s were derived from general requirements on tools for Kubernetes. Further requirements were derived from an inspection of the existing tools. Based on these requirements, the system design of Bunk8s was created and it was implemented in Go.

%Change to direct, remove a few

\end{abstract}

==> sections/04_evaluation.tex <==
% \section{Evaluation}
% \label{sec:evaluation}

% In this chapter, already existing tools that enable integration tests inside Kubernetes are compared to Bunk8s.

% \def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 

% % \begin{table}[t]
% % \centering
% % \begin{adjustbox}{width=\columnwidth,center}
% % \begin{tabular}{ |c||c|c|c|c| }
% %     \hline
% %     \multicolumn{5}{|c|}{Tool Comparison} \\
% %     \hline
% %      & \multicolumn{4}{c|}{Tool Name}\\
% %     \hline
% %     Feature & Bunk8s & Octopus \footnotemark & Istio \footnotemark & Jenkins \footnotemark \\
% %     \hline
% %     Broad integration testing & \checkmark{} & \checkmark{} & . & .\\
% %     Narrow integration testing & . & . & \checkmark{} & \checkmark{}\\
% %     Test framework independency & \checkmark{} & \checkmark{} & . & \checkmark{}\\
% %     Infrastructure independency & \checkmark{} & \checkmark{} & . & .\\
% %     Test result publishing & \checkmark{} & . & \checkmark{} & \checkmark{}\\
% %     \hline
% % \end{tabular}
% % \end{adjustbox}
% % \caption{Comparison of Bunk8s with other testing tools}
% % \label{table:comparison}
% % \end{table}

% \begin{table}[t]
% \centering
% \begin{adjustbox}{width=9cm,center}
% \begin{tabu}{ |c|c|c|c|c| }
%     \hline
%     \textbf{Supported Features} & \textbf{Bunk8s} \textbf{[This Work]} & \textbf{Octopus}  & \textbf{Istio}  & \textbf{Jenkins}  \\
%     \tabucline{-}
%     Broad integration testing & \faThumbsOUp & \faThumbsOUp & \faThumbsDown & \faThumbsDown\\
%     \tabucline{-}
%     Narrow integration testing & \faThumbsDown & \faThumbsDown & \faThumbsOUp & \faThumbsOUp\\
%     \tabucline{-}
%     Test framework independent & \faThumbsOUp & \faThumbsOUp & \faThumbsDown & \faThumbsDown \\
%     \tabucline{-}
%     Infrastructure independent & \faThumbsOUp & \faThumbsOUp & \faThumbsDown & \faThumbsDown\\
%     \tabucline{-}
%     Test result publishing & \faThumbsOUp & \faThumbsDown & \faThumbsOUp & \faThumbsOUp\\
%     \tabucline{-}
% \end{tabu}
% \end{adjustbox}
% \caption{Comparison of the features supported by \emph{Bunk8s} with other available tools for integration testing. \faThumbsOUp Supported. \faThumbsDown No support. }
% \label{table:comparison}
% \end{table}


% \addtocounter{footnote}{1}
% \footnotetext{https://github.com/kyma-incubator/octopus}
% \addtocounter{footnote}{1}
% \footnotetext{https://github.com/istio/istio}
% \addtocounter{footnote}{1}
% \footnotetext{https://github.com/jenkinsci/jenkins}

% Table \ref{table:comparison} gives an overview of the comparison of Bunk8s with the integration testing approaches of other tools.

% \subsubsection{Integration testing}

% All approaches enable integration testing inside Kubernetes, however, a distinction must be made between narrow and broad integration tests. 
% With the approach that can be implemented by using Jenkins, only narrow integration tests can be run. Due to the Istio sidecar container for pods, narrow integration tests can also be performed with Istio's test framework. Octopus, as well as Bunk8s, do not support narrow integration testing, but broad integration testing, which is the kind of integration tests that solves the problem with testing microservices as described in \autoref{sec:intro}. 

% % Narrow integration testing of containerized microservices can be performed outside of Kubernetes and does not require a deployment of services under test to a cluster. As soon as a test also covers a modules interaction with a module inside another service or public cloud infrastructure, it would be labeled as a broad integration test. 

% \subsubsection{Test framework independency}

% All tools are independent of a test framework, except for the Istio test framework. It requires developers to write tests with Go's default test package. Bunk8s allows developers to write tests in their preferred language or use a test framework, that is suited best for testing a given domain. 

% \subsubsection{Infrastructure independency}

% The Istio Test Framework is dependant on the use of Prow as CI/CD system in order to run integration tests. Since Jenkins is also a CI/CD tool, both approaches to integration testing may require the introduction of new CI/CD tools instead of allowing integration into already existing tools. The introduction would also come with the downside of increasing complexity, while Bunk8s can be used with any CI/CD tool, that supports running docker containers.

% \subsubsection{Test result publishing}

% Octopus does not support test result publishing since test results are not extracted from the test runners.
% Bunk8s supports test result publishing, since the test results are extracted from the test runner pod and are stored on the pipeline runner. Then the pipelines mechanisms for test result publishing can be used. This makes it uncomplicated to integrate Bunk8s into an existing projects pipeline. As previously mentioned, Istio, as well as Jenkins would require the introduction of new CI/CD tools in order to be integrated into an existing project.
